Classical 5D fields generated by a uniformly accelerated point source

Gauge fields associated with the manifestly covariant dynamics of particles in $(3,1)$ spacetime are five-dimensional. In this paper we explore the old problem of fields generated by a source undergoing hyperbolic motion in this framework. The 5D fields are computed numerically using absolute time $\tau$-retarded Green-functions, and qualitatively compared with Maxwell fields generated by the same motion. We find that although the zero mode of all fields coincides with the corresponding Maxwell problem, the non-zero mode should affect, through the Lorentz force, the observed motion of test particles.

==> UAP_specification.tex <==
%%
%% File   : UAP_specification.tex
%% Purpose: Define the uniform acceleration, 
%%          derive the fields, in integral forms, associated with it,
%%          and describe the numerical techniques needed to solve it.
%%
%%\subsection{Uniform acceleration in relativistic dynamics}
The motion of a source in hyperbolic motion follows a worldline 
given by
\begin{align}
    z^{\alpha}(\tau)
    & = 
        \dfrac{1}{g}
        \left\{
            \sinh(g\tau)
            ;
            0
            ,
            0
            ,
            \cosh(g\tau)
            ,
            \tau
        \right\}
\end{align}
where $g$ is the Newtonian acceleration in the local comoving inertial frame
\begin{align*}
    g & = \dfrac{d^2 (z^{3})}{d(z^{0})^2} \Big|_{\text{lf}} = \text{const.}
\end{align*}

In particular, this motion is \emph{on-shell}, as 
\begin{math}
    \dot{z}^2(\tau)
    = 
        -1
\end{math}

Thus, $R(\tau')$ now becomes
\begin{align*}
    R(\tau')
    & = 
        - \sigma_{5} x^2 
        +
        \dfrac{2 \sigma_{5}}{g}
        \left(
            x \cosh(g\tau')
            - 
            t \sinh(g\tau')
        \right)
        +
        \sigma_{5} (\tau - \tau')^2
\end{align*}
Thus, $R(\tau')$ is only \emph{linear} in the hyperbolic functions $\cosh(g\tau')$ or $\sinh(g\tau')$.

In the remaining of the paper, we shall limit the discussion to the case of $(4,1)$ metric, namely, $\sigma_{5} = +1$.
The reason behind this is the fact that for the $(4,1)$ case, support of the GF is in the \emph{5D timelike} region, which
seems more adequate when the Maxwell limit is taken.

However, it should be emphasized that the \emph{$(3,1)$ Maxwell-Einstein on-shell motion} of the source 
corresponds to the \emph{$(4,1)$ lightlike} motion, and therefore, would result in attaining special singular values 
along characteristics of the support of the GF's. This is similar to certain divergent regions in the field generated by 
a lightlike moving particle in Maxwell electrodynamics.

(Major outline:
\begin{itemize}
 \item Discuss conditions for regularizability - namely, the conditions when $R(\tau'_{0}) = \dot{R}(\tau'_{0}) = 0$ as well.
       Explain that this amounts to a shockwave front, and thus, the singularity is to be expected.
       Discuss similar problems in Maxwell electrodynamics.
 \item Discuss source motion region and its affect on regularization.
 \item Show that fields are generally not zero - there is no special frame for this problem.
 \item Discuss that the fields are form invariant under Lorentz boosts along the $\vb{\hat{z}}$ axis.
 \item Finally, show that any source undergoing acceleration experiences radiation reaction.
\end{itemize}
)

Numerical outline:
\begin{itemize}
 \item Discuss general outline of numerical solution.
       ($x-t-\rho$ space time grid, motion in $\tau$).
 \item Discuss how the roots of $R(\tau') = 0$ were found.
 \item 
\end{itemize}


